A two stages Deep Learning Architecture for Model Reduction of Parametric Time-Dependent Problems

Parametric time-dependent systems are of a crucial importance in modeling real phenomena, often characterized by non-linear behaviors too. Those solutions are typically difficult to generalize in a sufficiently wide parameter space while counting on limited computational resources available. As such, we present a general two-stages deep learning framework able to perform that generalization with low computational effort in time. It consists in a separated training of two pipe-lined predictive models. At first, a certain number of independent neural networks are trained with data-sets taken from different subsets of the parameter space. Successively, a second predictive model is specialized to properly combine the first-stage guesses and compute the right predictions. Promising results are obtained applying the framework to incompressible Navier-Stokes equations in a cavity (Rayleigh-Bernard cavity), obtaining a 97% reduction in the computational time comparing with its numerical resolution for a new value of the Grashof number.

==> sections/problem.tex <==

\section{Rayleigh-B\'{e}nard cavity flow}\label{section:cavity}

In order to extend our tests to larger systems, we present here the Rayleigh-B\'{e}nard cavity flow: a benchmark example that has been introduced in \cite{Roux:GAMM} and widely used since then, for example in \cite{Gelfgat:Ref11}, \cite{PR15} and \cite{HessQuainiRozza_ACOM_2022}. It considers the incompressible Navier-Stokes equations in a rectangular cavity. In particular, the model describes an important process in  semiconductor crystal growth \cite{KAKIMOTO1995191}, as it models the flow in the molten semiconductor material.

\subsection{Model description}

The incompressible Navier-Stokes equations describe viscous, Newtonian flow 
in the computational domain $\Omega \subset \mathbb{R}^d$. 
The unknowns are the vector field velocity $\bm u$ and scalar field pressure $p$. The incompressible Navier-Stokes equations are given as
\begin{eqnarray}\label{NS-1}
\frac{\partial {\bm u}}{\partial t}+({\bm u}\cdot  \nabla {\bm u})-\nu\Delta {\bm u}+\nabla p={\bm f} &\qquad\mbox{in } \Omega\times(0,T],\\ \label{NS-2}
\nabla \cdot {\bm u}=0&\qquad\mbox{in } \Omega\times (0,T].
\end{eqnarray}

\noindent where the kinematic viscosity is denoted $\nu$, the body forcing $\bm f$, and time interval as $T$. %denotes the time interval. 
The spatial dimension is either $d=2$ or $d=3$, while boundary and initial conditions are provided as
\begin{eqnarray}
{\bm u}={\bm u}_0&\qquad&\mbox{in } \Omega \times \{0\}, \label{IC}\\
{\bm u}={\bm u}_D&\qquad&\mbox{on } \partial\Omega_D\times (0,T], \label{BC-D} \\
-p \bm n + \nu \frac{\partial {\bm u}}{\partial \bm n}= \bm g &\qquad&\mbox{on } \partial\Omega_N\times, (0,T], \label{BC-N}
\end{eqnarray}

where $\partial\Omega_D \cap \partial\Omega_N = \emptyset$ and $\overline{\partial\Omega_D} \cup \overline{\partial\Omega_N} =  \overline{\partial\Omega}$. Here, ${\bm u}_0$, ${\bm u}_D$, and $\bm g$ are given and $\bm n$ denotes the outward pointing unit normal vector on the boundary $\partial\Omega_N$. The boundary $\partial \Omega_D$ is called the Dirichlet boundary and $\partial \Omega_N$ the Neumann boundary.

Let $L^2(\Omega)$ denote the space of square integrable functions in $\Omega$ and $H^1(\Omega)$ the space of functions belonging to $L^2(\Omega)$ with weak first derivatives in $L^2(\Omega)$. 
Define the sets 
%
\begin{eqnarray}
{\bm V} &:=& \left\{ {\bm v} \in [H^1(\Omega)]^d:  {\bm v} = {\bm u}_D \mbox{ on }\partial\Omega_D \right\},  \\
{\bm V}_0 &:=& \left\{{\bm v} \in [H^1(\Omega)]^d:  {\bm v} = \boldsymbol{0} \mbox{ on }\partial\Omega_D \right\}. 
\end{eqnarray}
%
The variational form of \eqref{NS-1}--\eqref{BC-N} is given by: find $({\bm u},p)\in {\bm V} \times L^2(\Omega)$, with ${\bm u}$ satisfying the initial condition \eqref{IC}, such that
%
\begin{align}
&\int_{\Omega} \frac{\partial{\bm u}}{\partial t}\cdot{\bm v} \mathbf{x}+\int_{\Omega}\left({\bm u}\cdot\nabla {\bm u}\right)\cdot{\bm v} \mathbf{x}
+\nu \int_{\Omega}\nabla {\bm u}\cdot \nabla{\bm v} \mathbf{x}- \int_{\Omega}p\nabla \cdot{\bm v} \mathbf{x} \nonumber \\
&\hspace{3cm} =\int_{\Omega}{\bf f}\cdot{\bm v} \mathbf{x}  + \int_{\partial \Omega_N}{\bf g}\cdot{\bm v} \mathbf{x} ,
\qquad\forall\,{\bm v} \in {\bm V}_0, \label{eq:weakNS-1}\\
& \int_{\Omega}q\nabla \cdot{\bm u} \mathbf{x} =0, \qquad\forall\, q \in L^2(\Omega).  \label{eq:weakNS-2}
\end{align}
%
Consider as computational domain $\Omega$ the rectangle with aspect ratio 4, i.e., a rectangle of height 1 and length 4.
The whole boundary is a no-slip boundary, so that $\partial\Omega_D = \partial\Omega$ and $\bm u_D = 0$.
The body forcing ${\bm f}$ is given by
%
\begin{align}
    {\bm f} = (0, \text{Gr}\nu^2 x)^T, \label{eq_f_cavity}
\end{align}
%
\noindent where $x$ is the horizontal coordinate and Gr is the Grashof number.
The Grashof number is a dimensionless number that describes the ratio of the buoyancy to viscous forces. 
\subsection{Discretization}

The numerical discretization method employed is the spectral element method
 \cite{karniadakis1999spectral}, which uses high-order polynomial ansatz functions over a coarse mesh, see Fig.~\ref{fig:mesh_cavity}.
The time-stepping scheme is an IMEX scheme of order 2 (IMplicit-EXplicit, see
\cite{Guermond_Shen_VCS}, \cite{Karniadakis_Orszag_Israeli_splitting_methods}), which is a standard option of the used PDE solver \emph{Nektar++}\footnote{https://www.nektar.info/}.
\begin{figure}[h!]
    \centering
    \includegraphics[scale=.4]{images/SEM_cavity_mesh.png}
    \caption{\small The computational mesh of the cavity is composed of 24 rectangles.}
    \label{fig:mesh_cavity}
\end{figure}


Our numerical studies will focus on the parameter domain $\Theta = [100 \cdot 10^3, 150 \cdot 10^3]$, and a full-order solution is computed at $Gr = 150\cdot 10^3$ over a long time interval to ensure that the limit cycle is reached. Then, each solution of interest in the interval $[100 \cdot 10^3, 150 \cdot 10^3]$ is initialized with the solution at $Gr = 150\cdot 10^3$. 

The time step is set to $1 \cdot 10^{-6}$ and for the tests $5 \cdot 10^{5}$ time steps have been computed.

\newpage

\subsection{Model order reduction}\label{POD}

Our Model Order Reduction technique aims to reduce
the cost of the full order solution computation by breaking it into two parts: a computationally expensive \emph{offline phase}, and a computationally efficient \emph{online phase}.

Indeed, the offline phase is the most time consuming because it comprehends both the collection of the full order solutions, and the training of the two stages architecture with these. On the other hand, the online phase is intended to be particularly fast, as it consists only in the computation of the first exact window $W_{new}$ and in the iterative time-step prediction by the framework (see Section \ref{architecture}).

Recalling what has been already analyzed in the ODE case in section~\ref{section:ODE}, the number of time-steps $w$ belonging to the time-window has an influence on the accuracy of the predictions, as a lower one, in general, implies a stronger error propagation. Despite of this, in the case of high-dimensional models, the computation of a long initial exact window can be as time consuming as the iterative prediction phase. Therefore, a compromise has to be made.

Moreover, to further reduce the order of the model, previous operations are performed on the full order solutions. 

In the first place, the velocity field solutions at every time step in the time interval of interest $T$, which are real vectors of high dimension $N$ ($N$
referring to size of the spatial discretization), are projected on a lower dimensional space through the Proper Orthogonal Decomposition approach (POD). It consists in finding a certain number of POD modes that reduces the dimension of the \emph{snaphots matrix} $\mathbf{S} = [\mathbf{s}_1,\dots,\mathbf{s}_T]$ (being $[\mathbf{s}_1,\dots,\mathbf{s}_T]$ the $T$ $N$-dimensional full order solutions). Such basis are computed through the Singular Value Decomposition of $\mathbf{S}$: $$\mathbf{S} = \mathbf{U}\mathbf{\Sigma}\mathbf{V^T},$$ where the columns of the unitary matrix $\mathbf{U}$ are the POD modes, and the diagonal matrix $\mathbf{\Sigma}$ contains the corresponding singular values in decreasing order. Considering only the first $N_{POD}$ rows of $\mathbf{U}$ according to the error we are willing to commit, we obtain the reduced order representation: $$\mathbf{S_{POD}} =  \mathbf{U_{N_{POD}}^T}\mathbf{S}.$$

In second place, because of the very small time-step required by the cavity simulations, in the collection of the training data-set for the two stages architecture only $1$ every $100$ time-steps is considered, so that also the online phase is accelerated having a larger prediction step.



%paper
%2 paragraphs
